Beyond the Margin: Targeted Conservation and Household Water Demand

Non-price interventions targeting specific household water uses are increasingly central to conservation policy, but whether end-use savings translate into lower aggregate demand remains unclear. This paper reports evidence from a pre-registered field experiment in which 775 Finnish households were randomized to a shower timer, a water-saving shower head, or the same shower head with real-time feedback. Utility-grade water meters measure household-level effects, while shower-level data provide complementary end-use evidence for the two shower-head treatments. The shower timer has no detectable effect. In contrast, the water-saving shower head reduces daily household demand by about 5%, and pairing it with real-time feedback doubles this reduction to about 10%. The convergence between shower- and meter-based estimates shows that end-use savings are consistent with limited offsetting elsewhere in the home. Cost-benefit analysis indicates that combining technological constraint with salient point-of-use feedback dominates reminder-based strategies.

==> Tables/tab_water_heterogeneity_pre_reg.tex <==
\begin{table}[H]\centering\scriptsize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{7}{cc}}
\hline\hline
          &\multicolumn{3}{c}{One tenant}&&\multicolumn{3}{c}{Multi tenant}\\
          \cline{2-4} \cline{6-8}
          &\multicolumn{1}{c}{Total}&\multicolumn{1}{c}{Cold}&\multicolumn{1}{c}{Hot}&&\multicolumn{1}{c}{Total}&\multicolumn{1}{c}{Cold}&\multicolumn{1}{c}{Hot}\\
\hline
\textit{H} &1.431 (3.18)         &0.610 (2.00)         &0.821 (1.47)      &   &0.733 (6.41)         &-3.298 (4.00)         &4.031 (3.25)         \\
\textit{SNoF} &-12.01\sym{**} (4.31)         &-7.233\sym{**} (2.27)         &-4.779\sym{*} (2.34)     &    &-2.325 (8.34)         &0.635 (5.72)         &-2.961 (3.33)         \\
\textit{SF} &-12.87\sym{**} (4.40)         &-6.145\sym{**} (2.32)         &-6.722\sym{**} (2.46)    &     &-20.06\sym{*} (7.76)         &-9.736\sym{*} (4.72)         &-10.33\sym{**} (3.59)         \\
Constant    &132.6\sym{***} (1.29)         &82.75\sym{***} (0.73)         &49.89\sym{***} (0.67)   &      &256.0\sym{***} (3.39)         &163.2\sym{***} (2.20)         &92.82\sym{***} (1.54)         \\
\hline
$\hat\beta_{1} = \hat\beta_{2}$&  0.00523         &  0.003         &   0.027      &   &    0.703         &    0.456         &   0.050         \\
$\hat\beta_{1} = \hat\beta_{3}$&  0.003         &   0.012         &  0.004      &   &  0.006         &    0.123         & 0.000         \\
$\hat\beta_{2} = \hat\beta_{3}$&    0.880         &    0.705         &    0.543    &     &   0.053         &   0.077         &   0.057         \\
$\hat\beta_{3} < \hat\beta_{2}$ & 0.440 & 0.648 & 0.272 & & 0.027 & 0.039 & 0.029\\
\midrule
Households&      345         &      345         &      345         &  &    188         &      188         &      188         \\
Observations&    27,600         &    27,600         &    27,600     &    &    15,040         &    15,040         &    15,040         \\
\hline\hline
\end{tabular}
  \caption{Heterogeneity of interventions effects. The three leftmost columns report the estimated coefficients for one-tenant households. The three rightmost columns for households with more than one tenant. Standard errors clustered at the household level in parentheses. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\).}
  \label{tab:meter_read_heterogeneity_pre_reg}
\end{table}


